An Empirically Fast Las Vegas Algorithm for Algebraic Shifting

Improved algorithms for computing (partial and full) exterior algebraic shifts of hypergraphs and simplicial complexes are presented. The main benefit is in positive characteristic. Experiments with an implementation in OSCAR with various inputs such as bipartite graphs and triangulations of two and three dimensional manifolds show that the method considerably extends for which simplicial complexes exterior algebraic shifts can be computed in practice.

==> definitions.tex <==
\makeatletter
\usepackage{mathtools,bm,microtype,calc,array,pdfpages,nicematrix,blkarray,tikz,tikz-cd,booktabs,hyphenat,csquotes,hyperref,cleveref,multirow,expl3,xparse}
\RequirePackage{biblatex}
\usepackage[flushmargin]{footmisc} % Remove footnote indentation
\graphicspath{{visualizations/}}
\renewbibmacro{in:}{, }
\DeclareFieldFormat[misc]{title}{\mkbibquote{#1}}
\DeclareFieldFormat{eprint:projecteuclid}{Project Euclid: \href{http://projecteuclid.org/euclid.#1}{\nolinkurl{#1}}}
%\DeclareFieldFormat[article]{volume}{\mkbibbold{#1}}
%\DeclareFieldFormat{url}{\textsc{url}: \href{#1}{#1}}
%\DeclareFieldFormat{doi}{\textsc{doi}: \href{http://dx.doi.org/#1}{#1}}
%\DeclareFieldFormat{eprint:arxiv}{arXiv:\href{https://arxiv.org/abs/#1}{#1}}
\addbibresource{biblio.bib}

%\usepackage{hyperref,cleveref}

% This patch accounts for a bug recently introduced in latex, see https://tex.stackexchange.com/q/730148/27717
\newcommand\patchtheorem[2]{\AddToHook{env/#1/begin}{\crefalias{#2}{#1}}}
\patchtheorem{lemma}{theorem}
\patchtheorem{proposition}{theorem}
\patchtheorem{corollary}{theorem}
\patchtheorem{conjecture}{theorem}
\patchtheorem{assumption}{theorem}
\patchtheorem{observation}{theorem}
\patchtheorem{example}{theorem}
\patchtheorem{definition}{theorem}
\patchtheorem{remark}{theorem}
\patchtheorem{question}{theorem}
\patchtheorem{problem}{theorem}

% Enable sub-theorems and references to them
\usepackage[patch-newtheorem]{mytheorem-enum}

\crefname{equation}{}{}
\Crefname{page}{page}{Pages}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{remark}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{example}[theorem]{Example}

\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{problem}[theorem]{Problem}

\newtheorem{claim}{Claim}[theorem]
\renewcommand{\theclaim}{\arabic{claim}}
\newtheorem*{claim*}{Claim}

\newenvironment{claimproof}[1][\proofname\ of Claim]{%
	\par\normalfont\topsep6\p@\@plus6\p@\relax
	\trivlist
	\item[\hskip\labelsep\itshape#1\@addpunct{.}]\ignorespaces
}{\endtrivlist\@endpefalse}


\Crefname{example}{Example}{Examples}
\Crefname{theorem}{Theorem}{Theorems}
\Crefname{lemma}{Lemma}{Lemmas}
\Crefname{proposition}{Proposition}{Propositions}
\Crefname{figure}{Figure}{Figures}
\Crefname{remark}{Remark}{Remarks}
\Crefname{corollary}{Corollary}{Corollaries}
\Crefname{conjecture}{Conjecture}{Conjectures}

\usepackage{xspace}
\newcommand\OSCAR{\texttt{OSCAR}\xspace}
\newcommand\polymake{\texttt{polymake}\xspace}
\newcommand\Macaulay{\texttt{Macaulay2}\xspace}

%\newcommand\doi[1]{\href{http://dx.doi.org/#1}{\texttt{doi:#1}}}

\newcommand\CC{{\mathbb C}}
\newcommand\EE{{\mathbb E}}
\newcommand\LL{{\mathbb L}}
\newcommand\NN{{\mathbb N}}
\newcommand\KK{{\mathbb K}}
\newcommand\PP{{\mathbb P}}
\newcommand\QQ{{\mathbb Q}}
\newcommand\RR{{\mathbb R}}
\newcommand\Sph{{\mathbb S}}
\newcommand\TT{{\mathbb T}}
\newcommand\ZZ{{\mathbb Z}}
\newcommand\FF{{\mathbb F}}

\newcommand\cD{{\mathcal D}}
\DeclareMathOperator{\Gin}{gin}
\DeclareMathOperator{\In}{in}
\newcommand\frM{{\mathfrak m}}
\newcommand\frR{{\mathfrak r}}
\newcommand\frU{{\mathfrak u}}
\newcommand\frV{{\mathfrak v}} % was previously defined in the middle of the main tex
\newcommand\frX{{\mathfrak x}}
\newcommand\frY{\mathfrak{y}}
\let\xto\xrightarrow
\let\symdiff\bigtriangleup
\newcommand{\Matr}{\mathcal{M}}
\DeclareMathOperator{\argmin}{arg\,min}
\DeclareMathOperator{\rk}{rk}
\newcommand\GF[1]{\operatorname{GF}(#1)}
\newcommand{\GL}{\mathrm{GL}}
\newcommand{\PSL}{\mathrm{PSL}}
\DeclareMathOperator{\Gr}{Gr}
\DeclarePairedDelimiterXPP{\SymmetricGroup}[1]{\operatorname{Sym}}{(}{)}{}{#1}
\newcommand{\PG}{\mathrm{PG}}
\DeclareMathOperator{\inv}{Inv}
\DeclareMathOperator{\card}{card}
\newcommand{\RepVert}[3]{#1|_{#2}^{#3}}
\newcommand{\NinLSpan}[2]{\mathrm{LLI}(#1, #2)}
\newcommand{\lex}[1]{#1_{\text{\rm lex}}}
\newcommand{\InitialSegment}{\mathrm{In}}
\newcommand{\ShiftGraph}{\mathrm{PSG}}
\newcommand{\ContractedGraph}{\overline{\ShiftGraph}}
\newcommand{\CShift}{\Gamma}
\DeclareMathOperator{\Char}{char}
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\actson}{\mathbin{\rotatebox[origin=c]{-90}{$\circlearrowleft$}}}
\newcommand{\actsfrom}{\mathbin{\rotatebox[origin=c]{90}{$\circlearrowright$}}}

% Set builder notation. Call by \Set{v; P(v)}, \Set*{v; P(v)} for auto-sized delimiters, or \Set[\big]{v; P(v)} for fixed size.
\DeclarePairedDelimiterX{\Set}[1]{\{}{\}}{\setargs{#1}}

% Linear span. Like \Set. Optionally takes the field as subscript; e.g., \Span_{k}*{v} or \Span_{k}[\big]{v}$.
\NewDocumentCommand{\Span}{E{_}{{}}}{\operatorname{span}_{#1}\SpanX}

% Use as \abs{}, \abs*{} or \abs[\big]{}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
% Internals for the above
\DeclarePairedDelimiterX{\SpanX}[1]{(}{)}{\setargs{#1}}
\NewDocumentCommand{\setargs}{>{\SplitArgument{1}{;}}m}{\setargsaux#1}
%\NewDocumentCommand{\setargsaux}{mm}{\IfNoValueTF{#2}{#1}{#1\nonscript\:\delimsize\vert\allowbreak\nonscript\:\mathopen{}#2}}%
\NewDocumentCommand{\setargsaux}{mm}{\IfNoValueTF{#2}{#1}{#1:\allowbreak #2}}%

% Small-script case distinction environment.
\newenvironment{smallcases}{\left\{\begin{smallmatrix*}[l]}{\end{smallmatrix*}\right.}

% Cases with brace on both sides (https://tex.stackexchange.com/a/308762/27717)
\newcases{lrcases}{\quad}
{$\m@th\textstyle{##}$\hfil}
{$\m@th\textstyle{##}$\hfil}
{\lbrace}
{\rbrace}
\newcases{lrdcases*}
{\quad}
{$\m@th\textstyle{##}$\hfil}
{{##}\hfil}
{\lbrace}
{\rbrace}

% Align in substack (https://tex.stackexchange.com/a/198806/27717)
\newcommand{\subalign}[1]{%
	\vcenter{%
		\Let@ \restore@math@cr \default@tag
		\baselineskip\fontdimen10 \scriptfont\tw@
		\advance\baselineskip\fontdimen12 \scriptfont\tw@
		\lineskip\thr@@\fontdimen8 \scriptfont\thr@@
		\lineskiplimit\lineskip
		\ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\hfil\crcr
			#1\crcr
		}%
	}%
}

% Produce command \MakeCommaBreakable that makes comma breakable in inline math (https://tex.stackexchange.com/a/716369/27717.
{
	\gdef\OldComma{,}
	\catcode`\,=13
	\gdef\MakeCommaBreakable{%
		\catcode`\,=13
		\def,{%
			\ifmmode
			\OldComma\>\allowbreak
			\else
			\OldComma
			\fi
		}%
	}
}

% Small version of array (https://tex.stackexchange.com/a/98692/27717)
\newenvironment{smallarray}[1]{%
	\null\,\vcenter\bgroup\scriptsize%
	\renewcommand{\arraystretch}{0.7}%
	\arraycolsep=.13885em%
	\hbox\bgroup$\array{@{}#1@{}}%
}{%
	\endarray$\egroup\egroup\,\null%
}

% Scaling version of \vdots and \ddots (better than mathdots package, see https://tex.stackexchange.com/a/246695/27717)
\usepackage{letltxmacro}
\LetLtxMacro\orgvdots\vdots
\LetLtxMacro\orgddots\ddots
\DeclareRobustCommand\vdots{%
	\mathpalette\@vdots{}%
}
\newcommand*{\@vdots}[2]{%
	% #1: math style
	% #2: unused
	\sbox0{$#1\cdotp\cdotp\cdotp\m@th$}%
	\sbox2{$#1.\m@th$}%
	\vbox{%
		\dimen@=\wd0 %
		\advance\dimen@ -3\ht2 %
		\kern.5\dimen@
		% remove side bearings
		\dimen@=\wd2 %
		\advance\dimen@ -\ht2 %
		\dimen2=\wd0 %
		\advance\dimen2 -\dimen@
		\vbox to \dimen2{%
			\offinterlineskip
			\copy2 \vfill\copy2 \vfill\copy2 %
		}%
	}%
}
\DeclareRobustCommand\ddots{%
	\mathinner{%
		\mathpalette\@ddots{}%
		\mkern\thinmuskip
	}%
}
\newcommand*{\@ddots}[2]{%
	% #1: math style
	% #2: unused
	\sbox0{$#1\cdotp\cdotp\cdotp\m@th$}%
	\sbox2{$#1.\m@th$}%
	\vbox{%
		\dimen@=\wd0 %
		\advance\dimen@ -3\ht2 %
		\kern.5\dimen@
		% remove side bearings
		\dimen@=\wd2 %
		\advance\dimen@ -\ht2 %
		\dimen2=\wd0 %
		\advance\dimen2 -\dimen@
		\vbox to \dimen2{%
			\offinterlineskip
			\hbox{$#1\mathpunct{.}\m@th$}%
			\vfill
			\hbox{$#1\mathpunct{\kern\wd2}\mathpunct{.}\m@th$}%
			\vfill
			\hbox{$#1\mathpunct{\kern\wd2}\mathpunct{\kern\wd2}\mathpunct{.}\m@th$}%
		}%
	}%
}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% % % preliminary version only
%\usepackage[colorinlistoftodos,bordercolor=orange,backgroundcolor=orange!20,linecolor=orange,textsize=tiny]{todonotes}
%\usepackage{prelim2e}
%\renewcommand{\PrelimText}{\raisebox{-\height}[0pt][0pt]{\sf\scriptsize --- INCOMPLETE DRAFT of \today ---}}
%\setlength{\marginparwidth}{1.2in}

%% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Make \text{\todo{...}} work in math; see https://tex.stackexchange.com/a/132451/27717
% Michael: I do not like it, because this code does not correctly separate overlapping boxes
%\usepackage{marginnote}
%\makeatletter
% \renewcommand{\@todonotes@drawMarginNoteWithLine}{%
	% 	\begin{tikzpicture}[remember picture, overlay, baseline=-0.75ex]%
		% 		\node [coordinate] (inText) {};%
		% 	\end{tikzpicture}%
	% 	\marginnote[{% Draw note in left margin
		% 		\@todonotes@drawMarginNote%
		% 		\@todonotes@drawLineToLeftMargin%
		% 	}]{% Draw note in right margin
		% 		\@todonotes@drawMarginNote%
		% 		\@todonotes@drawLineToRightMargin%
		% 	}%
	% }

\newlength\ExtraCaptionMargin

% Footnote without number
\newcommand\blfootnote[1]{%
	\begingroup
	\renewcommand\thefootnote{}\footnote{#1}%
	\addtocounter{footnote}{-1}%
	\endgroup
}

\newcommand{\Email}[1]{\href{mailto:#1}{#1}}

\let\origDdots\ddots
\renewcommand{\ddots}[1][0]{\mathpalette\ddotsI{#1}}
\newcommand{\ddotsI}[2]{\rotatebox[origin=c]{#2}{$#1\origDdots$}}

\newcommand\SwapBelowDisplaySkip{\vskip-\belowdisplayskip\vskip\belowdisplayshortskip\noindent}

% Separates multiple citations by semicolon, rather than comma
\renewcommand\multicitedelim{\addsemicolon\space}

% From https://tex.stackexchange.com/a/19100
\mathchardef\breakingcomma\mathcode`\,
{\catcode`,=\active
	\gdef,{\breakingcomma\discretionary{}{}{}}
}
\newcommand{\mathlist}[1]{$\mathcode`\,=\string"8000 #1$}

% Create a new columntype A[fmt] := S[table-format=fmt]
\makeatletter
\newtoks\mytoks
\mytoks\expandafter{\the\NC@list}
\newcolumntype{A}{}
\NC@list\expandafter{\the\mytoks \NC@do A}
\renewcommand*{\NC@rewrite@A}[1][]{%
	\@temptokena\expandafter{%
		\the\@temptokena
		S[table-format=#1]
	}%
	\NC@find
}
\makeatother

% Create a new columntype M[fmt] := S[table-format=fmt]
\makeatletter
\newtoks\mytoks
\mytoks\expandafter{\the\NC@list}
\newcolumntype{M}{}
\NC@list\expandafter{\the\mytoks \NC@do M}
\renewcommand*{\NC@rewrite@M}[1][]{%
	\@temptokena\expandafter{%
		\the\@temptokena
		S[round-mode=places, round-precision=0, fixed-exponent=9, scientific-notation=fixed, drop-exponent, table-format=#1]
	}%
	\NC@find
}

\makeatother

